Learning with Episodic Hypothesis Testing in General Games: A Framework for Equilibrium Selection

We introduce a new hypothesis testing-based learning dynamics in which players update their strategies by combining hypothesis testing with utility-driven exploration. In this dynamics, each player forms beliefs about opponents' strategies and episodically tests these beliefs using empirical observations. Beliefs are resampled either when the hypothesis test is rejected or through exploration, where the probability of exploration decreases with the player's (transformed) utility. In general finite normal-form games, we show that the learning process converges to a set of approximate Nash equilibria and, more importantly, to a refinement that selects equilibria maximizing the minimum (transformed) utility across all players. Our result establishes convergence to equilibrium in general finite games and reveals a novel mechanism for equilibrium selection induced by the structure of the learning dynamics.

==> game_definition.tex <==
\section{Model and Preliminaries}\label{sec: model}

\subsection{The static game model}

We consider a static game \( G = (I, A = (A_i)_{i \in I}, (u_i)_{i \in I}) \), where:
\begin{itemize}
    \item \( I \) is a finite set of players, with \( |I| = n \),
    \item \( A_i \) is a finite set of actions for player \( i \), and \( A := \prod_{i \in I} A_i \) denotes the set of joint action profiles. Let \( A_{-i} := \prod_{j \ne i} A_j \) denote the set of joint actions of players other than \( i \),
    \item \( u_i : A \to \mathbb{R} \) is the payoff function for player \( i \).
\end{itemize}

For each player \( i \), a mixed strategy \( \pi_i = (\pi_i(a_i))_{a_i \in A_i} \in \Delta_i \) is a probability distribution over \( A_i \), where \( \Delta_i \) denotes the simplex on \( A_i \). A joint strategy profile is \( \pi = (\pi_i)_{i \in I} \in \Delta := \prod_{i \in I} \Delta_i \), the space of joint mixed strategies. The expected utility for player \( i \) under \( \pi \) is:
\[
U_i(\pi) = \mathbb{E}_{a \sim \pi}[u_i(a)].
\]
We next define the smooth best response function and the \(\epsilon\)-Nash equilibrium.

\begin{definition}[Smooth Best Response]
For any player \( i \in I \) and temperature parameter \( \sigma > 0 \), the smooth best response function \( \Br_i^\sigma : \Delta_{-i} \to \Delta_i \) is defined by:
\begin{align}\label{eq:smoothed_br}
    \Br_i^\sigma(a_i \mid \pi_{-i}) = \frac{e^{U_i(a_i, \pi_{-i})/\sigma}}{\sum_{a_i' \in A_i} e^{U_i(a_i', \pi_{-i})/\sigma}}, \quad \forall a_i \in A_i, \quad \forall \pi_{-i} \in \Delta_{-i}.
\end{align}
The joint smooth best response function \( \Br^\sigma : \Delta \to \Delta \) is:
\[
\Br^\sigma(\pi) = (\Br_i^\sigma(\pi_{-i}))_{i \in I}.
\]
\end{definition}

\begin{definition}[\(\epsilon\)-Nash Equilibrium]
For any \( \epsilon > 0 \), a strategy profile \( \pi^* \in \Delta \) is an \(\epsilon\)-Nash equilibrium if:
\[
U_i(\pi_i^*, \pi_{-i}^*) \ge U_i(\pi_i', \pi_{-i}^*) - \epsilon, \quad \forall \pi_i' \in \Delta_i, \quad \forall i \in I.
\]
As \( \epsilon \to 0 \), \( \pi^* \) becomes a Nash equilibrium.
\end{definition}



\subsection{Discretized belief and hypothesis testing} 
Each player \( i \) holds a \emph{belief} \( b_i \) of the joint strategy profile of all players other than themselves, and a belief profile is $b = (b_i)_{i \in I}$. Let \( \Delta_i^M \) denote the \emph{discretized probability simplex} for player \( i \) with granularity parameter \( M \in \mathbb{N}_{+} \):
% \[
% \Delta_i^M := \left\{ \pi_i(a_i) \in \mathbb{R}^{|A_i|} \;\middle|\; \sum_{a_i \in A_i} \pi_i(a_i) = 1,\; \pi_i(a_i) \in \left\{ \frac{m}{M} : m = 0,\ldots,M \right\},\; \pi_i(a_i) \ge 0 \right\}.
% \]
\[
\Delta_i^M := \left\{ \pi_i(a_i) \in \mathbb{R}^{|A_i|}_{\geq 0} \;\middle|\; \sum_{a_i \in A_i} \pi_i(a_i) = 1,\; \pi_i(a_i) \in \left\{ \frac{m}{M} : m = 0,\ldots,M \right\} \right\}.
\]
We define the \emph{discretized belief space} $
\mathcal{B}_i := \prod_{j \ne i} \Delta_j^M$, and the \emph{joint discretized belief space} for all players is $\mathcal{B} := \prod_{i \in I} \mathcal{B}_i$. A hypothesis test evaluates whether player \( i \)'s belief \( b_i \) is close to the true strategy profile $\pi_{-i}$ of all players other than $i$. Given a tolerance level $\tau > 0$, we define:

\begin{itemize}
    \item[-] The null hypothesis \( H_0 \): The strategy profile $\pi_{-i}$ is within $\tau$-distance to player \( i \)'s belief $b_i$:
    \[ \|\pi_{-i} - b_i\|_2 \leq \tau .\]
    \item[-] The alternative hypothesis \( H_1 \): The strategy profile $\pi_{-i}$ is not within $\tau$-distance to player \( i \)'s belief $b_i$:
    \[ \|\pi_{-i} - b_i\|_2 > \tau .\]
\end{itemize}

For each player $i$, let $\{a_{-i}^t\}_{t=1}^{T}$ be $T$ independent and identically distributed (i.i.d.) action samples draws from their opponents strategy profile $\pi_{-i}$. The goal of player $i$ is to design a hypothesis test that controls the probability of Type I and Type II errors:
\begin{itemize}
    \item[] \textbf{Type I error} (false positive): rejecting \( H_0 \) even though it is true ($\|\pi_{-i}-b_i\|_2\leq\tau$).
    \item[] \textbf{Type II error} (false negative): failing to reject \( H_0 \) even though \( H_1 \) is true ($\|\pi_{-i}-b_i\|_2>\tau$).
\end{itemize}
%We fix a \emph{significance level} \( \bar{\alpha} \in (0,1) \), representing the maximum allowable probability of a Type I error.


The following proposition analyze the type I and type II error of all hypothesis tests. The proof is provided in Appendix \ref{appendix: proof of hypothesis test}.
\begin{proposition} \label{prop: hypothesis test}
    For any $\bar{\alpha} \in (0,1)$, suppose that each player $i$ rejects $H_0$ if and only if 
    \begin{align*}
        L_T = \|\hat{\pi}_{-i} - b_i \|_2 > \tau  + \sqrt{\frac{|A_{-i}|}{2T}\cdot\ln\bigl(\tfrac{2}{\bar\alpha}\bigr)}, 
    \end{align*}
    where $\hat{\pi}_{-i}$ is the empirical distribution of strategy profile for all players other than $i$:
\[
  \hat{\pi}_{-i}(a_{-i}) =
  \frac{1}{T}\sum_{t=1}^{T}\mathbf1\{a_{-i}^{t} = a_{-i}\}, 
  \qquad \forall a_{-i}\in A_{-i}.
\]
Then, given sample size \[T(\bar{\alpha})\geq \max_{\substack{i \in I,\\ \pi_{-i}, b_i \in \mathcal{B}_i,\\\|\pi_{-i}-b_i\|_2 > \tau}}\frac{2|A_{-i}|}{(\|\pi_{-i} - b_i\|_2-\tau)^2}\,\ln\bigl(\frac{2}{\bar{\alpha}}\bigr),\] the type I error rate and type II error rate of the test are upper bounded by $\bar{\alpha}$ for all players, i.e.  
\begin{align*}
&\sup_{\{b_i \in \mathcal{B}_i, \pi_{-i} \in \Delta_{-i}:~  \|b_i - \pi_{-i}\|_2 \leq \tau\}} P(\text{reject } H_0| b_i,\pi_{-i}) \leq \bar{\alpha}, \quad \forall i \in I, \\
& \sup_{\{b_i \in \mathcal{B}_i, \pi_{-i} \in \Delta_{-i}:~ \|b_i - \pi_{-i}\|_2 > \tau\}} P(\text{fail to reject } H_0| b_i,\pi_{-i}) \leq \bar{\alpha}, \quad \forall i \in I. 
\end{align*}
\end{proposition}



% Let $Z^\dagger$ be the belief states:
% From lemma \ref{lemma: tau, best response}, for any $z = (b, \pi) \in Z^\dagger$, and any $i \in I$, $\pi_i$ is an $\epsilon$-best response to all other players' strategy $\pi_{-i}$. Therefore, each state $z = (b, \pi) \in Z^\dagger$ corresponds to an $\epsilon$-stationary Nash equilibrium.


% For the remainder of this paper, we assume that for any chosen \(\epsilon>0\), the parameters \(M\), \(\tau\), and \(\sigma\) satisfy Assumption~\ref{assump: sigma, tau, M}. For simplicity, we refer to a \((\tau, \sigma)\)-consistent state \(z^*\) simply as a consistent state. From Lemma~\ref{lemma: sigma, tau, M}, we know that the strategy profile in any consistent state constitutes an \(\epsilon\)-Nash equilibrium.

% at least one belief $b \in \mathcal{B}_i$ that is $\tau$-consistent. That is, 
%     let $\pi = \Br^{\sigma}(b)$, then for all $i \in I$,
%     \begin{align*}
%         \|b_i - \pi_{-i}\|_2 \leq \tau.
%     \end{align*}
    % Furthermore, for any $\tau$-consistent belief $b \in \mathcal{B}$, $\pi = \Br^{\sigma}(b)$ is an 
% \manxi{Introduce discretization of $\Delta$ space, introduce belief in this discretized space, smoothed best response $BR$. 
% A belief is $\tau$-consistent is (insert $H_0$ condition). One assumptions: (i) assumption about the condition of $\tau$ given $\epsilon$. (ii) assumption about $M$ given $\epsilon$. (iii) $\sigma$. 
% Lemma: For any $\epsilon$, suppose Assumption holds, the strategy profile induced by the smoothed best response of belief is an $\epsilon$-Nash equilibrium if belief is $\tau$-consistent and it is nonempty.}

%The following Lemma shows that for any $\epsilon > 0$, there exists a choice of temperature parameter $\sigma$, tolerance $\tau$, and discretization granularity $M$ such that there exists at least one $\tau$-consistent belief $b \in \mathcal{B}$. Furthermore, for any $\tau$-consistent belief $b \in \mathcal{B}$, the induced smooth response strategy $\pi = \Br^{\sigma}(b)$ an $\epsilon$-Nash equilibrium. We postpone the proof to Appendix \ref{appendix: large M}.

%We refer to the tuple \(z= (b, \pi)\), where \(b \in \mathcal{B}\) and \(\pi \in \Delta\), as the \emph{state} of the system. %We denote the set of all states as $Z= \mathcal{B} \times \Delta$. %
% \begin{definition}
%     For any $\tau>0$ and $\sigma>0$, a state \(z= (b, \pi)\) is $(\tau, \sigma)$-consistent if 
%     \begin{itemize}
%         \item[(i)] the $\ell_2$ distance between belief $b_i$ and strategy profile $\pi_{-i}$ is smaller than or equal to $\tau$ for all players:  
%     \[ \|\pi_{-i} - b_i\|_2 \leq \tau, \quad \forall i \in I.\]
%     \item[(ii)] each player's strategy is a smooth best response to their belief with temperature parameter $\sigma$, i.e. $\pi_i = \Br_i^\sigma(\pi_{-i})$ for all $i \in I$. 
%     \end{itemize}
% \end{definition}

%  




% \paragraph{The static game model.} We consider a static game $G=(I, A = (A_i)_{i \in I}, (u_i)_{i \in I})$, where:
% \begin{itemize}
%     \item $I$ is a finite set of players, with $|I| = n$.
%     \item $A_i$ is a finite set of actions for each player $i \in I$. Let $A := \prod_{i \in I} A_i$ be the set of joint action profiles, and  $A_{-i} := \prod_{j \neq i} A_i$ be the set of joint action profiles for all players other than $i$.
%     \item $u_i: A \rightarrow \mathbb{R}$ is a payoff function for each player $i \in I$.
% \end{itemize}

% For each player $i \in I$, a mixed strategy $\pi_i = (\pi_i(a_i))_{a_i \in A_i}\in \Delta_i$ is a probability distribution over $A_i$, where $\Delta_i$ denotes the probability simplex on $A_i$. A joint strategy profile is denoted by $\pi := (\pi_i)_{i \in I} \in \Delta = \prod_{i \in I} \Delta_i$, where $\Delta$ is the set of joint mixed strategies. 
% %Let $\Delta_i$ be the probability simplex on action space $A_i$, \(\Delta:= \prod_{i \in I} \Delta_i\) be the simplex space for joint strategy profiles, and \(\Delta_{-i}:= \prod_{j I \setminus \{i\}} \Delta_j\) be the simplex space for joint strategy profiles for all players other than $i$. For each player $i \in I$, a strategy $\pi_i \in \Delta_i$ specifies the probability $ \pi_i(a_i) $ of choosing action $a_i$. 
% %The joint strategy profile of all players is $\pi := (\pi_i)_{i \in I} \in \Delta$. Similarly, $\pi_{-i} := (\pi_j)_{j \in I \setminus \{i\}} \in \Delta_{-i}$ is the joint strategy of all players except $i$.  
% Given a strategy profile $\pi$, the expected utility for each player $i \in I$ is $\U{i}{\pi} = \mathbb{E}_{a \sim \pi} \left[u_i(a)\right]$. We next define the smooth best response function and the $\epsilon$-Nash equilibrium. 
% \begin{definition}
% For any player $i \in I$ and temperature parameter $\sigma>0$, define the smooth best response function $\Br^{\sigma}_i: \Delta_{-i} \to \Delta_i$ by %be the smooth response function with temperature \( \sigma > 0 \). For any strategy profile $\pi_{-i} \in \Delta_{-i}$, the smooth response strategy $\Br^{\sigma}_i(b_i): A_i \to [0,1]$ chooses any action $a_i \in A_i$ with probability:
% \begin{align*}
%     \Br^{\sigma}_i(a_i| \pi_{-i}) = 
%     \frac{e^{U_i(a_i, \pi_{-i})/\sigma}}{\sum_{a'_i \in A_i} e^{U_i(a'_i, \pi_{-i})/\sigma}}, \quad \forall a_i \in A_i, \quad \forall \pi_{-i} \in \Delta_{-i}.
% \end{align*}
% The joint smooth best response function is given by $\Br^{\sigma}(\pi) = (\Br^{\sigma}_i(\pi_{-i}))_{i \in I}$. 
% \end{definition}

% \begin{definition}
% Given any $\epsilon > 0$, a strategy profile $\pi^* \in \Delta$ is an $\epsilon$-Nash equilibrium if %for all player $i \in I$, strategy $\pi^*_i$ is an $\epsilon$-best response to $\pi^*_{-i}$, i.e. 
% \[
% \U{i}{\pi^*_i, \pi^*_{-i}} \geq \U{i}{\pi'_i, \pi^*_{-i}} - \epsilon, \quad \forall \pi'_i \in \Delta_i, ~ \forall i \in I. 
% \]As $\epsilon \to 0$, $\pi^{*}$ is a Nash equilibrium.
% \end{definition}


%Moreover, for any $\pi_{-i}$, we define a smooth best response function of player $i$ as $\Br^{\sigma}_i: \Delta_{-i} \to \Delta_i$.
% \ruifan{change $b_i$ to $\pi_{-i}$}


% \color{blue} 

% Road Map:
% \begin{enumerate}
%     \item define logit response function $\Br^{\sigma}_i(b_i)$
%     \item existence of fixed point belief and strategy
%     \item logit response function is Lipschitz in $U$ and $b$
%     \item Given small enough $\sigma$, the logit response strategy is an $\epsilon/2$-best response. [$\sigma$ depends on $\epsilon$.]
%     \item Let $\pi = \Br^{\sigma}(b)$. Given smaller enough $\tau$, if for all $i \in I$, $\|b_i - \pi_{-i}\|_2 \leq \tau$, then $\pi$ is an $\epsilon$-equilibrium. [$\tau$ depends on $\epsilon$ and $\sigma$.]
%     \item Given large enough $M$, there exist $b$ in the discretized space $\Delta^M$ such that if $\pi = \Br^{\sigma}(b)$, we have  $\|b_i - \pi_{-i}\|_2 \leq \tau$ for all $i \in I$. [$M$ depends on $\tau$ and $\sigma$.]
% \end{enumerate}

% \color{black}




% \begin{lemma}  %\label{lemma: large M}
%     For any $\epsilon>0$, suppose that the discretization parameter $M$ satisfies 
% \begin{align}%\label{eq: granularity M}
%         M \geq \max_{i \in I}\frac{|A_i| \cdot 2L \cdot |I|}{\epsilon},
%     \end{align}
%     where 
%     \begin{align*}
%         L = \max_{i \in I, a \in A} |u_i(a)|,
%     \end{align*}
%     then for any player $i$ and any opponents' strategy \(\pi_{-i} \in \Delta^M_i\), there exists an \(\epsilon\)-best response strategy \(\tilde{\pi}_i\) in the discretized strategy space \(\Delta^M_i\). Furthermore, there exists an \(\epsilon\)-Nash equilibrium \(\tilde{\pi}^*_i\) in the discretized strategy space \(\Delta^M_i\). 
%     %That is, for all \(i \in I\) and for every strategy \(\pi'_i \in \Delta(A_i)\),\[
%     % \U{i}{\tilde{\pi}^*_i, \tilde{\pi}^*_{-i}} \geq \U{i}{\pi'_i, \tilde{\pi}^*_{-i}} - \epsilon.
%     % \]
%  \end{lemma}
% We defer the proof to appendix \ref{appendix: large M}. For the rest of the paper, we assume that $M$ satisfies \eqref{eq: granularity M} so that $\epsilon$-best response strategy and $\epsilon$-Nash equilibrium are well-defined and exist in $\Delta^M$ for our game. 
 

% \ruifan{existence of eta equilibrium, combine lemma 123, best response + Nash existence, define the eta Nash set on the grid with notation $NE$, use newcommand.}
% \manxi{You have a mixed Nash, and you round the strategy to the nearest one on the grid. Upper bound the utility difference for each player }\ruifan{done}

% \begin{lemma} \label{lemma: lipchitz}
%     For each $i \in i$, the expected payoff function \( \U{i}{\pi}\) is Lipschitz continuous in \(\pi\) with Lipschitz constant \(L = \max_{i \in I, a \in A} |u_i(a)|\).
% \end{lemma}
% \begin{proof}
%     Let \(\pi\) and \(\pi'\) be two strategy profiles in the continuous strategy simplex \(\Delta(A)\). We want to show that there exists a constant \(L > 0\) such that:
%     \[
%     |\U{i}{\pi} - \U{i}{\pi'}| \leq L \|\pi - \pi'\|_1,
%     \]
%     where \(\|\pi - \pi'\|_1\) is the \(L^1\) norm of the difference between \(\pi\) and \(\pi'\).
    
%     The expected payoff for player \(i\) under strategy \(\pi\) is:
%     \[
%     \U{i}{\pi} = \mathbb{E}_{a \sim \pi}[u_i(a)] = \sum_{a \in A} \pi(a) u_i(a).
%     \]
%     Therefore, the difference in expected payoffs satiesfies
%     \begin{align*}
%         |\U{i}{\pi} - \U{i}{\pi'}| &= \left|\sum_{a \in A} (\pi(a) - \pi'(a)) u_i(a)\right|\\
%         &\leq \sum_{a \in A} |\pi(a) - \pi'(a)| |u_i(a)|.
%     \end{align*}
%     % By the triangle inequality
    
%     Let \(L = \max_{i \in I, a \in A} |u_i(a)|\). Then,
%     \[
%     |\U{i}{\pi} - \U{i}{\pi'}| \leq L \sum_{a \in A} |\pi(a) - \pi'(a)| = L \|\pi - \pi'\|_1.
%     \]
    
%     Thus, \(\U{i}{\pi}\) is Lipschitz continuous in \(\pi\) with Lipschitz constant \(L\).
% \end{proof}

% \begin{lemma}
%     For any \(\epsilon > 0\), let granularity parameter $M$ be such that \[M \geq \max_{i \in I}\frac{|A_i| \cdot L}{\epsilon}.\] Then, for any strategy \(\pi_{-i} \in \Delta^M_i\), there exists a \(\epsilon\)-best response \(\pi_i\) in the discretized strategy space \(\Delta^M_i\).
%  \end{lemma}

%  \begin{proof}
%     Let \(\epsilon > 0, \pi_{-i} \in \Delta^M_i\) be arbitrary. Let $\pi^*_i$ be a best response in the continuous simplex $\Delta(A_i)$ such that for any $\pi'_i \in \Delta(A_i)$, we have 
%     \[
%     \U{i}{(\pi^*_i, \pi_{-i})} \geq \U{i}{(\pi'_i, \pi_{-i})}.
%     \]
%  Since granularity $M$ is sufficiently large
%     \[
%     M \geq \max_{i \in I}\frac{|A_i| \cdot L}{\epsilon},
%     \]
%     there exists $\pi_i$ such that for each $a_i \in A_i$, $\pi_i(a_i)$ are sufficiently close to $\pi^*_i(a_i)$ 
%     \[|\pi_i(a_i) - \pi^*_i(a_i)| \leq \frac{|A_i| \cdot L}{\epsilon}.\]
%     Hence the $L_1$ distance between $\pi^*_i$ and $\pi_i$ are sufficiently small:
%     \begin{align*}
%         \|\pi_i - \pi^*_i\|_1 &= \sum_{a_i \in A_i} |\pi_i(a_i) - \pi^*_i(a_i)|\\
%         &\leq \sum_{a_i \in A_i} \frac{\epsilon}{|A_i| \cdot L}\\
%         &= \frac{\epsilon}{L}.
%     \end{align*}
    
%     From lemma \ref{lemma: lipchitz}, the expected payoff function \(\U{i}{\pi}\) is Lipschitz continuous with constant \(L\), we have:
%     \[
%     |\U{i}{\pi_i, \pi_{-i}} - \U{i}{\pi^*_i, \pi_{-i}}| \leq L \|(\pi_i, \pi_{-i}) - (\pi^*_i, \pi_{-i})\|_1 = L \|\pi_i - \pi^*_i\|_1 \leq \epsilon.
%     \]

%     Therefore, for any \(\pi'_i \in \Delta(A_i)\), we have 
%     \[
%     \U{i}{\pi_i, \pi_{-i}} \geq \U{i}{\pi^*_i, \pi_{-i}} -\epsilon \geq \U{i}{\pi'_i, \pi_{-i}} - \epsilon.
%     \]

%     Thus, \(\pi_i\) is an \(\epsilon\)-best response to $\pi_{-i}$ in the discretized strategy space $\Delta^M_i$.
% \end{proof}


% \begin{lemma}
%     For any \(\epsilon > 0\), let granularity parameter $M$ be such that \[M \geq \max_{i \in I}\frac{|A_i| \cdot 2L \cdot |I|}{\epsilon}.\] 
%     There exists an \(\epsilon\)-Nash equilibrium \(\tilde{\pi}^*_i\) in the discretized strategy space \(\Delta^M_i\). 
%     That is, for all \(i \in I\) and for every strategy \(\pi'_i \in \Delta(A_i)\),
%     \[
%     \U{i}{\tilde{\pi}^*_i, \tilde{\pi}^*_{-i}} \geq \U{i}{\pi'_i, \tilde{\pi}^*_{-i}} - \epsilon.
%     \]
%  \end{lemma}

%  \begin{proof}
    
%     Let \(\epsilon > 0\) be arbitrary. From Nash's theorem, there exists a Nash equilibrium $\pi^*$ in the continuous simplex $\Delta(A)$ such that for any $i \in I, \pi'_i \in \Delta(A_i)$, we have 
%     \[
%     \U{i}{(\pi^*_i, \pi^*_{-i})} \geq \U{i}{(\pi'_i, \pi^*_{-i})}.
%     \]
%     Since granularity $M$ is sufficiently large
%     \[
%     M \geq \max_{i \in I}\frac{|A_i| \cdot 2L \cdot |I|}{\epsilon},
%     \]
%     for all $i \in I$, there exists $\tilde{\pi}_i$ such that for each $a_i \in A_i$, $\tilde{\pi}_i(a_i)$ are sufficiently close to $\pi^*_i(a_i)$ 
%     \[|\tilde{\pi}_i(a_i) - \pi^*_i(a_i)| \leq \frac{1}{M} \leq \frac{\epsilon}{|A_i| \cdot 2L \cdot |I|}.\]
%     Hence for any $i \in I$, the $L_1$ distance between $\pi^*_i$ and $\tilde{\pi}_i$ are sufficiently small:
%     \begin{align*}
%         \|\tilde{\pi}_i - \pi^*_i\|_1 &= \sum_{a_i \in A_i} |\tilde{\pi}_i(a_i) - \pi^*_i(a_i)|\\
%         &\leq \sum_{a_i \in A_i} \frac{\epsilon}{|A_i| \cdot 2L \cdot |I|}\\
%         &= \frac{\epsilon}{2L \cdot |I|}.
%     \end{align*}
    
%     From lemma \ref{lemma: lipchitz}, the expected payoff function \(\U{i}{\pi}\) is Lipschitz continuous with constant \(L\), we have:
%     \begin{align*}
%         |\U{i}{\tilde{\pi}} - \U{i}{\pi^*}| 
%         &\leq L \|\tilde{\pi} - \pi^*\|_1 \\
%         &= L \sum_{i \in I} \|\tilde{\pi}_i - \pi^*_i\|_1 \\
%         &\leq L \cdot \frac{\epsilon}{2L} \\
%         &\leq \frac{\epsilon}{2}.
%     \end{align*}

%     For any $\pi'_i \in \Delta(A_i)$,
%     \begin{align*}
%         |\U{i}{\pi'_i, \pi^*_{-i}} -  \U{i}{\pi'_i, \tilde{\pi}^*_{-i}}| & \leq L \cdot \|(\pi'_i, \pi^*_{-i}) - (\pi'_i, \tilde{\pi}^*_{-i})\|_1\\
%         &= L \cdot \sum_{j \neq i} \|\pi^*_j - \tilde{\pi}^*_j\|_1\\
%         &\leq L \sum_{j \neq i} \frac{\epsilon}{L \cdot |I|}\\
%         &\leq \frac{\epsilon}{2}
%     \end{align*}

%     Therefore, for any \(i \in I, \pi'_i \in \Delta(A_i)\), we have 
%     \[
%     \U{i}{\tilde{\pi}^*} \geq \U{i}{\pi^*} -\frac{\epsilon}{2} \geq \U{i}{\pi'_i, \pi^*_{-i}} - \frac{\epsilon}{2} \geq \U{i}{\pi'_i, \tilde{\pi}^*_{-i}} - \epsilon.
%     \]

%     Thus, \(\tilde{\pi}^*\) is an \(\epsilon\)-Nash equilibrium in the discretized strategy space $\Delta^M_i$.
% \end{proof}


 

% \manxi{$t$ or $k$? Also, I don't think this is the right place to introduce repeated interaction because you don't carry $k$ or $t$ in notation in the next section.} The game proceeds 
% % in epochs indexed by $k = \{1,2,\cdots\}$, and each epoch proceeds 
% in discrete-time stages indexed by $t \in \{1, 2,\dots \}$. 
% At each time step $t$, each player samples action $a_i^t$ from their current strategy $\pi_i$ (\manxi{Not indexed with $k$?}), forming the joint action profile $ a^t := (a_i^t)_{i \in I} $. 
% We assume that each player observes action profiles $a^t$ at each time step, and knows its reward function $u_i$ and transition function $P$ of the process.

==> hypothesis_test.tex <==

\section{Hypothesis testing}

We propose a learning algorithm based on hypothesis testing. Each player $i \in I$ holds a belief $b_{ij}\in \Delta^M_j$ on player $j$'s strategy. Let $b_i = (b_{ij})_{j \in I}$ be player $i$'s belief on strategy profile for all player $j \neq i$. Let $B_i = \prod_{j \neq i}\Delta^M_j$ be the set of all possible true strategy (\manxi{true strategy? not belief?}) profiles of all players other than $i$. Since the action space $A$ of the game is finite, and the discretized simplex $\Delta^M$ is finite, the number of all (\manxi{This is belief or what?}) possible strategy profiles $|B_i|$ is finite for each $i \in I$. Let $B = \prod_{i \in I} B_i$ be the set of all possible belief profile. (\manxi{This whole paragraph is confusing and unncessarily complicated.})

\begin{definition}
    A hypothesis test for player $i$ tests their belief $b_i$ against the observed action profiles. (\manxi{Did you read this sentence after writing it? Or did you use chatGPT to help you revise?}) Define the null hypothesis and the alternative hypothesis as follow:\\
    \indent $H_0$: The observed action profile are sampled from player $i$'s belief (\manxi{There is grammar mistake. Also, please use AI to revise.}): \[\pi_{-i} = b_i.\]
    \indent $H_1$: The observed action profile are not sampled from player $i$'s belief: \[\pi_{-i} \neq b_i.\]
    

    The null hypothesis $H_0$ is rejected if and only if the observed data fall into the reject region of the test. (\manxi{You have not defined the rejected region.})

    % $H_0$: Player $i$'s belief $b_i$ is accurate: \[\pi_j = b_{ij}, \quad \forall j \neq i, j \in I.\]
    % $H_1$: Player $i$'s belief $b_i$ is not accurate:
    % \[\pi_j \neq b_{ij}, \quad \text{ for some} j \neq i, j \in I.\]
    
    % If a hypothesis test starts at $\bart$, it will last for $\T$ periods, during which player $i$ plays according to their strategy $\pi_i$, and observes actions $a^{\bart}, \cdots, a^{\bart+\T}$. At the end of the hypothesis test, player $i$ will reject the null hypothesis $H_0$ or fail to reject $H_0$.
\end{definition}

\manxi{Use notation $H_0$ and $H_1$ in definitions.}
\begin{definition}
    The type I error rate $\alpha$ of a hypothesis test is the probability of rejecting the null hypothesis given that it is true. 
\end{definition}
\begin{definition}
    The type II error rate $\beta$ of a hypothesis test is the probability of failing to reject the null hypothesis given that the alternative hypothesis is true. The power ($1-\beta$) of a hypothesis test is the probability of correctly rejecting the null hypothesis given that the alternative hypothesis is true.
\end{definition}


\subsection{base test} \label{sec: base test}

\manxi{This paragraph should be placed later.} In this section, we show that for any player $i \in I$ with belief $b_i \in B_i$, player $i$ can conduct a hypothesis test with $\bart$ samples which has type I error rate \(\bara < 0.5\), and type II error rate \(\barb(b_i, \pi_{-i}, \bart) < 0.5\) for any true strategy profile $\pi_{-i} \in \Delta^M_{-i}$.

\manxi{Add paragraph tag The base test.} For any player $i \in I$ with any belief $b_i \in B_i$, let the base hypothesis test with significance level $\bara$ be defined as follow. Let $\pi_{-i} \in B_i$ be the true strategy profile for all player other than $i$. 
% The null hypothesis $H_0$ and alternative hypothesis $H_1$ is:\\
% \indent $H_0$: The observed action profile are sampled from player $i$'s belief: $\pi_{-i} = b_i$.\\
% \indent $H_1$: The observed action profile are not sampled from player $i$'s belief: $\pi_{-i} \neq b_i$.\\
Given $\TT$ samples from observed action profiles $a_{-i} \sim \pi{-i}$,  we can compute the chi-square test statistic: \[\chi_{b_i}^2 = \sum_{a \in A}\frac{(N(a_{-i}) - b_i(a_{-i})\cdot \TT)^2}{b_i(a_{-i})\cdot \TT},\]
where $N(a_{-i})$ is the actual observed number for $a_{-i}$ in the $\TT$ samples, and $b_i(a_{-i}) = \prod_{j \neq i, j \in I}b_{ij}(a_{j})$ is the expected probability of sampling action profile $a_{-i}$ given belief $b_i$. Player $i$ rejects the null hypothesis $H_0$ if and only if \[\chi_{b_i}^2 > \chi^2_{\bara, |A_{-i}|-1}.\]
\manxi{Is it clear what is $\chi^2_{\bara, |A_{-i}|-1}$. Also, $\chi_{b_i}^2$ is not a good notation, not distinguished from $\chi^2_{\bara, |A_{-i}|-1}$.}


\manxi{There are many issues with the next lemma so I used chatgpt to help me revise. Please adopt the notation in this version throughout the paper. 
\begin{lemma}Suppose player \( i \in I \) conducts a hypothesis test with \( T \) samples and significance level \( \bar{\alpha} \) to evaluate belief \( b_i \in B_i \) against the true strategy profile \( \pi_{-i} \). The Type I error rate of the test is \( \bar{\alpha} \), and the Type II error rate is:
\[
\bar{\beta}(b_i, \pi_{-i}, T, \bar{\alpha}) = 1 - F_{\chi^2_{d}(\lambda)}(\chi^2_{d, 1-\bar{\alpha}}),
\]
where:
\begin{itemize}
    \item[-] The noncentrality parameter \( \lambda \) is given by:
  \[
  \lambda = T \sum_{a_{-i} \in A_{-i}} \frac{(\pi_{-i}(a_{-i}) - b_i(a_{-i}))^2}{b_i(a_{-i})}.
  \]
\item[-] \( d = |A_{-i}| - 1 \) is the degrees of freedom, with \( A_{-i} = \prod_{j \neq i} A_j \) denoting the set of action profiles for all players except \( i \).
\item[-] \( F_{\chi^2_d(\lambda)}(x) \) is the CDF of a noncentral chi-square distribution with \( d \) degrees of freedom and noncentrality parameter \( \lambda \).
\item[-] \( \chi^2_{d, 1-\bar{\alpha}} \) is the critical value of the central chi-square distribution at significance level \( \bar{\alpha} \).
\end{itemize}
\end{lemma}
Maybe it is more clear to add the dependent variables to $\lambda$, up to you. }
\begin{lemma} \label{lemma: power of base test}
    For any player $i \in I$, belief $b_i \in B_i$, and true strategy profile $\pi_{-i}$, suppose player $i$ conduct a base hypothesis test with $\TT$ samples and significance level $\bara$. (\manxi{What is significance level and how is that different from the type I error rate?}) The type I error rate of the test is $\bara$. The type II error rate of the test is $\barb(b_i,\pi_{-i}, \TT, \bara)$, where
    \begin{align*}
        \barb(b_i,\pi_{-i}, \TT, \bara) &= 1- F_{\chi^2_{|A_{-i}|-1}(\lambda(\pi_{-i}, b_i, T))}(\chi^2_{\bara, |A_{-i}|-1}).
    \end{align*}
    In the above expression, $A_{-i} = \prod_{j \neq i, j \in I} A_j$ is the set of all possible action profiles by all players other than player $i$. $F_{\chi^2_{k}(\lambda)}$ (\manxi{Are you sure this is the right notation?}) is the CDF of a noncecntral (\manxi{what is this? Misspelled?}) chi-square distribution with $k$ degree of freedom and parameter $\lambda$. $\chi^2_{\bara,k}$ is the critical value for $\chi^2$ distribution with $k$ degree of freedom and significance level $\bara$. $\lambda(\pi_{-i}, b_i, T)$ is the noncecntral chi-square parameter: \[\lambda(\pi_{-i}, b_i, T) = \TT \sum_{a \in A} \frac{(\pi_{-i}(a_{-i}) - b_i(a_{-i}))^2}{b_i(a_{-i})}.\]
\end{lemma}
\begin{proof}\manxi{Please see my conversation with GPT on how to revise this proof. \url{https://chatgpt.com/share/67d0d80e-6cf8-800a-a3d3-2423e327fd42}}
    Let $i \in I, b_i \in B_i, \pi_{-i} \in \Delta^M_{-i}$ be arbitrary. The belief $b_i$ follows a multinomial distribution with $|A_{-i}|$ categories. Each action profile $a_{-i}$ has expected probability $b_i(a_{-i}) = \prod_{j \neq i, j \in I}b_{ij}(a_{j})$. Given $\TT$ samples, the expected observed counts for $a_{-i}$ is $b_i(a_{-i})\cdot \TT$. $N(a_{-i})$ is the actual observed count for $a_{-i}$. 
    Hence, the chi-square test statistic is: \[\chi_{b_i}^2 = \sum_{a \in A}\frac{(N(a_{-i}) - b_i(a_{-i})\cdot \TT)^2}{b_i(a_{-i})\cdot \TT}.\]
    If the null hypothesis $H_0$ is true, the test statistics $\chi_{b_i}^2$ follows a Chi-square distribution with $|A_{-i}|-1$ degree of freedom. Hence, the type I error rate is the probability of rejecting $H_0$ when $b_i = \pi_{-i}$:
    \[P(\chi_{b_i}^2 > \chi^2_{\bara, |A_{-i}|-1} \mid \pi_{-i} = b_i) = \bara.\]

    If the true strategy profile is $\pi_{-i} \neq b_i$, then the test statistics follows a noncentral Chi-square distribution $\chi^2_{|A_{-i}|-1}(\lambda(\pi_{-i}, b_i, T))$ with noncentral parameter:
    \[\lambda(\pi_{-i}, b_i, T) = \TT \cdot \sum_{a \in A} \frac{(\pi_{-i}(a_{-i}) - b_i(a_{-i}))^2}{b_i(a_{-i})}.\]

    Let $F_{\chi^2_{k}(\lambda)}$ be the CDF of a noncecntral chi-square distribution with $k$ degree of freedom and parameter $\lambda$. The type II error rate is the probability that we fail to reject $H_0$ when $\pi_{-i}$ is true:
    \begin{align*}
        \barb(b_i,\pi_{-i}, T, \bara) &=
        P(\chi_{b_i}^2 < \chi^2_{\bara, |A_{-i}|-1} \mid \pi_{-i})\\
        &= F_{\chi^2_{|A_{-i}|-1}(\lambda(\pi_{-i}, b_i, T))}(\chi^2_{\bara, |A_{-i}|-1}).
    \end{align*}
\end{proof}


\begin{lemma} \label{lemma: base test}
    \manxi{There exists some sample size (please use proper language)} We can find some sample size $\bart$ such that for any player $i \in I$, any belief $b_i \in B_i$, and any true strategy profile $\pi_{-i} \in \Delta^M_{-i}$, if player $i$ conducts a base test with $\bart$ sample size, it has type I error rate
    \[\bara < 0.5,\]
    and type II error rate
    \[\barb(b_i, \pi_{-i}, \bart) < 0.5.\]
\end{lemma}

\begin{proof}
    Let $i \in I, b_i \in B_i, \pi_{-i} \in \Delta^M_{-i}$ be arbitrary. Choose the significance level $\bara = 0.49$. From lemma \ref{lemma: power of base test}, we know the type II error rate with $\TT$ samples is:
    \begin{align*}
        \barb(b_i,\pi_{-i}, T, \bara) &=
        P(\chi_{b_i}^2 < \chi^2_{\bara, |A_{-i}|-1} \mid \pi_{-i})\\
        &= F_{\chi^2_{|A_{-i}|-1}(\lambda(\pi_{-i}, b_i, T))}(\chi^2_{\bara, |A_{-i}|-1})\\
        &= 1- Q_{(|A_{-i}|-1)/2}(\sqrt{\lambda(\pi_{-i}, b_i, T)}, \sqrt{\chi^2_{\bara, |A_{-i}|-1}}),
    \end{align*}
    where $Q$ is the Marcum Q function.

    Notice that $\lambda(\pi_{-i}, b_i, T)$ goes to infinity as the sample size $\TT$ increases:
    \[\lim_{\TT \to \infty}\lambda(\pi_{-i}, b_i, T) = \lim_{\TT \to \infty} \TT \cdot \sum_{a \in A} \frac{(\pi_{-i}(a_{-i}) - b_i(a_{-i}))^2}{b_i(a_{-i})} = \infty.\]
    Since for any $u > 0, v \geq 0$, the Marcum Q-function approches $1$ as its first parameter approches infinity:
    \[\lim_{x \to \infty} Q_u(x, v) = 1,\]
    we have the type II error rate approches $0$ as the sample size $\TT$ approaches infinity:
    \begin{align*}
        &\quad \lim_{\TT \to \infty} \barb(b_i,\pi_{-i}, T, \bara) \\
        &= \lim_{\TT \to \infty} 1- Q_{(|A_{-i}|-1)/2}(\sqrt{\lambda(\pi_{-i}, b_i, T)}, \sqrt{\chi^2_{\bara, |A_{-i}|-1}})\\
        &= 0.
    \end{align*}

    Hence, there exists $\bart > 0$ such that
    \[\min_{i \in I, b_i \in \Delta^M_i, \pi_{-i} \neq b_i \in \Delta^M_i} \barb(b_i,\pi_{-i}, \bart, \bara) < 0.5.\] That is, we can find $\bart$ such that for any player $i$, any belief $b_i$, and any true strategy $\pi_{-i}$, the base test has type I error $\bara = 0.49 < 0.5$ and type II error $\barb(b_i,\pi_{-i}, \bart) := \barb(b_i,\pi_{-i}, \bart, \bara) < 0.5$.
\end{proof}



\subsection{powerful test}

We can generate arbitrarily accurate hypothesis tests using some relatively accurate base tests. Take a base hypothesis test with sample size $\bart$ and type I error $\bara < 0.5$ and type II error $\barb < 0.5$. For any \(T\) rounds of data collected, partition the data into \(\lfloor T/\bart \rfloor\) disjoint subsets, each containing \(\bart\) elements, disregarding any remaining elements. If \(\lfloor T/\bart \rfloor\) is even, discard the last subset of size \(\bart\). Subsequently, perform the base hypothesis test on each of the remaining subsets of size \(\bart\). The null hypothesis is rejected if and only if it is rejected by the original test on a majority of these subsets.


\begin{lemma}[\cite{Foster2003}] \label{lemma: power test from base test}
    Given a base hypothesis test with sample size $\bart$ and type I error $\bara < 0.5$ and type II error $\barb < 0.5$, the ensembled hypothesis test has sample size $T$ and type I error rate $\alpha$ and type II error rate $\beta$ satisfying:
    \[\alpha \leq s_0e^{-l_0T}, \quad \beta \leq s_0e^{-l_0T},\]
    where \[s_0 = \max(\bara(4\bara(1-\bara))^{-2},\barb(4\barb(1-\barb))^{-2}),\] 
    and \[l_0 = \min(\frac{\log(4\bara(1-\bara))}{2\bart},\frac{\log(4\barb(1-\barb))}{2\bart}).\]
\end{lemma}

Proposition \ref{prop: hypothesis test} shows that for any player $i \in I$ with belief $b_i \in B_i$, we can use the above procedure and the base test described in section \ref{sec: base test} to construct a hypothesis with arbitraily small type I and type II error rate.

\begin{proposition} \label{prop: hypothesis test}
    Let $\epsilon, r_0$ be arbitrary. Let $\bart$ be the sample size of the base tests described in section \ref{sec: base test}, and let $\bara$ be the type I error rate, $\barb(b_i, \pi_{-i}, \bart)$ be the type II error rate for player $i$ with belief $b_i$ and true strategy $\pi_{-i}$. Let
    \begin{align*}
        s &= \max_{\substack{i \in I, b_i \in \Delta^M_i, \\\pi_{-i} \neq b_i \in \Delta^M_i}}(\bara(4\bara(1-\bara))^{-2},\barb(b_i, \pi_{-i}, \bart)(4\barb(b_i, \pi_{-i}, \bart)(1-\barb(b_i, \pi_{-i}, \bart)))^{-2}),\\
        l &= \min_{\substack{i \in I, b_i \in \Delta^M_i, \\\pi_{-i} \neq b_i \in \Delta^M_i}}(\frac{\log(4\bara(1-\bara))}{2\bart},\frac{\log(4\barb(b_i, \pi_{-i}, \bart)(1-\barb(b_i, \pi_{-i}, \bart)))}{2\bart}).
    \end{align*} 
    For any player $i \in I$ with belief $b_i \in B_i$, and true strategy profile $\pi_{-i} \in \Delta^M_{-i}$, the ensembled hypothesis test with sample size $T(\epsilon)$:
    \[T(\epsilon) =  -\frac{1}{l}\ln(\epsilon^{r_0}/s),\]
    has type I error rate: \[\alphai \leq \epsilon^{r_0},\] 
    and type II error rate: \[\betai \leq \epsilon^{r_0}.\] 
\end{proposition}
% \ruifan{In fact, a sufficient condition for the errors is $\alphai \leq \epsilon^{r_0}$ and $\beta_i \to 0$. There is no requirement for the rate of decay for type ii error rate.}




\begin{proof}
    Let $\epsilon, r_0$ be arbitrary. Let $i \in I, b_i \in B_i, \pi_{-i} \in \Delta^M_{-i}$ be arbitrary. From lemma \ref{lemma: base test}, the base hypothesis test with sample size $\bart$ has type I error rate $\bara$ and type II error rate $\barb(b_i, \pi_{-i}, \bart)$:
    \[\bara < 0.5, \quad \barb(b_i, \pi_{-i}, \bart) < 0.5.\]
    From lemma \ref{lemma: power test from base test}, we can use the base test to construct an ensembled hypotheis test with sample size $\T$, type I error rate $\alphai$ and type II error rate $\betai$:
    \[\alphai \leq s_0e^{-l_0\T}, \quad \betai \leq s_0e^{-l_0\T},\]
    where
    \begin{align*}
        s_0 &= \max(\bara(4\bara(1-\bara)^{-2},\barb(b_i, \pi_{-i}, \bart)(4\barb(b_i, \pi_{-i}, \bart)(1-\barb(b_i, \pi_{-i}, \bart)))^{-2}),\\
        l_0 &= \min(\frac{\log(4\bara(1-\bara))}{2\bart},\frac{\log(4\barb(b_i, \pi_{-i}, \bart)(1-\barb(b_i, \pi_{-i}, \bart)))}{2\bart}).
    \end{align*}
    Since $s_0 \leq s$ and $l_0 \geq l$, we have
    \[\alphai \leq se^{-l\T}, \quad \betai \leq se^{-l\T}.\]
    Since 
    \[T(\epsilon) =  -\frac{1}{l}\ln(\epsilon^{r_0}/s),\]
    we have 
    \begin{align*}
        \alphai &\leq se^{-l\T}\\
        &= s e^{-l \cdot (-\frac{1}{l}\ln(\epsilon^{r_0}/s))}\\
        &= s e^{(r_0\ln(\epsilon) - \ln(s))}\\
        &= \epsilon^{r_0}.
    \end{align*}
    Similarly, 
    \begin{align*}
        \betai \leq \epsilon^{r_0}.
    \end{align*}
\end{proof}





% \begin{proposition}
%     Let $\epsilon$ be arbitrary. Suppose a hypothesis test for player $i$ is rejected if and only if the empirical strategy for any player $j$, $\hat{\pi}_{j}$ is at least $\tau$ away from player $i$'s belief $b_{ij}$ about player $j$'s strategy:
%     \begin{align*}
%         \|\hat{\pi}_j - b_{ij}\| > \tau.
%     \end{align*}
%     With sufficiently large $\T$, and sufficiently small $\tau$, the hypothesis test has type I error smaller than $\epsilon$ and type II error smaller than $\epsilon$. (need to be further formalized)
% \end{proposition}

% \ruifan{explore test starting prob $\frac{1}{\T} + \tc$}

==> introduction.tex <==

\section{Introduction}

Although there is a rich literature on decentralized learning for repeated games, most convergence guarantees either apply only to specific game classes (e.g., zero-sum or potential games) or ensure convergence only to weak limiting equilibria such as correlated equilibrium (CE). Moreover, when equilibria are non-unique, their equilibrium outcome can differ drastically. Consequently, it remains open whether one can design decentralized learning algorithms that (i) converge to a Nash equilibrium in general finite games and (ii) offer equilibrium selection according to social welfare.

In this paper, we propose a learning dynamics with following properties:
\begin{enumerate}[(1)]
    \item \textbf{Belief-based}: Each player holds a belief over the mixed strategy profile about all players other than themselves. 
    \item \textbf{Smooth best response}: Each player always plays a smooth best response to their belief.
    \item \textbf{Episodic hypothesis testing}: Occasionally, each player conduct hypothesis test to check if the observed plays are consistent with current belief.
    \item \textbf{Utility-driven exploration:} Each player, even when the observed plays are consistent with their belief, might resample a new belief with a probability proportionate to their expected utility: the lower the expected utility, the higher the probability of exploration.
\end{enumerate}

Our main result shows that, under these dynamics, at least $1-\epsilon$ of the time, the actual strategy profiles being played consist of an $\epsilon$-Nash equilibrium that maximizes the minimum value of the function \( f_i(\U{i}{\pi}) \) over all players $i \in I$ is maximized. Formally, we prove that the learning dynamics consist of a Markov process with finite belief-strategy space, and the stochastically stable states of the Makrov process are:
\begin{itemize}
    \item \textbf{Consistent}: the belief profile are close to the actual strategy profile being played. Since each player smooth best response to their belief, the actual strategy profiles being played are $\epsilon$-Nash equilibrium.
    \item \textbf{The fairest equilibrium}: the strategy profile maximizes the minimum utility across all players.
\end{itemize}

The key insight driving this equilibrium selection is that the statistical hypothesis testings preserve belief accuracy and Nash stability of strategy profile, while utility-driven exploration biases learning toward regions of the strategy space that yield higher worst-case payoffs. Together, these ingredients create a natural mechanism for equilibrium selection, without external coordination or central control. 

Analyzing this rule presents several technical challenges. First, we present hypothesis tests with sufficiently small Type I and II error rates when the sample size/epoch length of the learning dynamics are sufficiently large.  Second, we showed that learning dynamics induce a high-dimensional Markov chain on the joint belief-strategy state space. Lastly, we apply Young's \cite{Young1993}'s framework of analyzing \textit{stochastically stable states} and show that
\begin{itemize}
    \item The learning dynamics induces a class of Markov chain that is a \textit{regular perturbation} of the limiting Markov chain where the Type I and Type II error rates and the exploration probabilities vanishes.
    \item The recurrence classes of the limiting Markov chain are induced by the \textit{belief consistent states} where the belief profile are close to the actual strategy profile.
    \item When the type I and type II error rate are sufficiently small, the \textit{stochastic potential} of each consistent state is governed by the exploration probability of the player with the smallest expected utility. Hence, the \textit{stochastically stable states} are the consistent states that that maximize the minimum utility across players.
\end{itemize}

The remainder of the paper is organized as follows. Section \ref{sec: model} introduces the game-theoretic model, beliefs, and hypothesis tests. Section \ref{sec:algo} introduces the learning algorithm and provides the convergence result by analyzing the stochastically stable set, and Section \ref{section: proof of main theorem} contains the proofs of the main results.

\paragraph{Literature Review}
Extensive research has examined the convergence properties of a wide array of learning dynamics in games. One strand of this literature study learning dynamics in which each player holds a belief about the opponent's strategies, and plays a best response strategy to their belief. In fictitious play and joint strategy fictitious play (\citet{Fudenberg1998}, \citet{marden2009c}), the belief consists of the empirical frequencies of opponents’ actions. However, fictitious play only converges to the Nash equilibrium for special classes of games, such as zero-sum games, dominance-solvable games, and potential games.
\citet{Kalai1993} study Bayesian updating, where players hold prior beliefs about their opponents’ strategies, and update those beliefs via Bayes’ rule. They show that the learning process will converge to an $\epsilon$-equilibrium of the repeated game if the learning rule satisfies the ‘grain-of-truth’ assumption: the initial beliefs must be compatible with the eventual play. However, several impossibility theorems (\citet{FosterYoung2001}, \citet{Nachbar1997, Nachbar2005, Nachbar2001}) suggest that it is difficult to find such learning rules. \citet{Foster1997} study on calibrated forecasting, where empirical frequencies of action profiles match players' beliefs in the long run. They propose a randomized calibration rule and prove that, when players best respond myopically to their calibrated forecasts, the population converges to the set of correlated equilibria. \citet{Kakade2004} present a weakly calibrated forecasting rule and show that the actual play converges to the set of $\epsilon$-Nash equilibria, and the joint empirical frequency converges to the convex hull of a set of $\epsilon$-Nash equilibria. \citet{Mannor2007} present a weakly calibrated forecasting rule that is memory-efficient, and provide conditions under which convergence to Nash equilibria may occur. 

Our work extends the class of learning rules where players update their beliefs through hypothesis testing. In \citet{Foster2003}, players hold beliefs about their opponents’ play and take the best responses. If they find that their hypothesis is wrong, then they randomly choose a new hypothesis of how their opponents play. They show that the play is $\epsilon$ close to being a subgame perfect equilibrium (SPE) at least ($1-\epsilon$) of the time. None of the above work provide equilibrium selection results. \citet{Jindani2022} extends the hypothesis testing learning rule by adding an exploration phase, where players may choose to sample new beliefs even if their current hypotheses are correct. He shows that for two-player games, this learning rule selects a subgame-perfect equilibrium of the repeated game in which payoffs are Pareto efficient. In contrast, our convergence result extends to multi-player games.

Another branch of literature focuses on learning rules that do not build a model for opponents, but rather learning the payoff of different actions directly. \citet{Hart2000} study regret matching and show almost sure convergence of the empirical frequencies of play to the set of correlated equilibria. However, regret matching still requires players to observe the action profile being played. Studying learning rules that do not depend on opponents’ actions or payoffs, \citet{Foster2006} and \citet{Germano2007} introduce regret testing, in which players play their intended strategies mostly and experiment occasionally. They periodically evaluate the regret of their intended strategies with some fixed action, and choose a new strategy if their original strategies perform badly. If every player plays according to it, the mixed action profiles converge almost surely to a Nash equilibrium of the stage game. \citet{Young2009} introduces interactive trial and error learning, where each player maintains a benchmark action, payoff, and moods (content, hopeful, watchful, or discontent); and performs mood-driven experimentation and updates. Under this learning scheme, the actual play converges to Nash equilibria in any game with generic payoffs and at least one pure Nash equilibrium. However, equilibrium selection remains unaddressed in these approaches.

Several literature study the problem of selecting socially optimal equilibrium outcomes. \citet{Marden2009a, Marden2009b}, \citet{MardenShamma2012} study log-linear learning, in which each player experiments with a small probability and adopts actions according to a logit function of their payoffs. For potential games, this learning rule selects potential maximizing action profiles. \citet{Pradelski2012} propose a learning procedure that combines ideas from both trial and error with log-linear learning. This procedure selects an efficient pure Nash equilibrium in any game with generic payoffs where pure Nash equilibria exist. When such equilibria do not exist, this procedure converges to action profiles that maximize a linear combination of the sum of payoffs across all agents and the payoff gain that would result from a deviation by some agent. \citet{MardenYoungPao2012} study a similar algorithm that converges to a Pareto efficient action profile for any game. Using similar structure with mood-driven trial-and error with small‐probability experimentation, \citet{Marden2017} and \citet{Borowski2019} develop learning dynamics where players' period-by-period joint strategies constitutes an welfare-maximizing coarse correlated equilibrium (CCE) with high probability. These welfare-maximizing learning rules either only guarantee convergence to a potential-maximizing action profile regardless of Nash stability, or only converge within the set of pure NE or CCE. 
In contrast, our algorithm ensures convergence within the  Nash equilibria set while selecting the equilibrium that maximizes the minimum utility across players. 





==> learning_with_episodic_hypothesis_testing.tex <==
\section{Learning dynamics and stochastically stable set}\label{sec:algo}

Algorithm~\ref{alg:learning with hypothesis testing} describes a learning process where players periodically test their beliefs about other players' strategies and resample new beliefs of opponents. We begin by outlining the overall structure of the learning process, before detailing the key quantities that govern the algorithm’s dynamics.

In Algorithm~\ref{alg:learning with hypothesis testing}, each player $i$ begins with an initial belief $b_i^0$ about others’ strategies and selects a smoothed best response strategy $\pi_i^0$ corresponding to their belief, as in \eqref{eq:smoothed_br}. The learning proceeds in \emph{epochs} ($k=1,2,\ldots$). In each epoch $k$, each player $i$ maintains belief $b_i^k$ and plays the game according to a smoothed best response strategy $\pi_i^k$ for $T(\xi^{\bar{r}})$ rounds, collecting observations of joint action profiles. Here, $\xi \in (0,1)$ is a hyperparameter of the learning dynamics.
Each player $i$ may independently decide whether to conduct a hypothesis test against their current belief $b_i^k$, with probability $\gamma(\xi) > 0$. The hypothesis test is as defined in Proposition \ref{prop: hypothesis test}, with $\xi^{\bar{r}}$ as the significance level and $T(\xi^{\bar{r}})$ as the sample size. If the null hypothesis is rejected (indicating a significant discrepancy between the observed actions and belief $b_i^k$), player $i$ samples a new belief $b_i^{k+1}$ uniformly from the belief space and updates their strategy to the corresponding best response $\pi_i^{k+1} = \mathrm{Br}_i^\sigma(b_i^{k+1})$. If the null hypothesis is not rejected, player $i$ may still sample a new belief (referred to as exploration) with probability $\xi^{f_i(U_i(\pi^k_i,b^k_i))}$. If neither testing nor exploration occurs, the player does not update their belief and strategy. 


\begin{algorithm}[ht]
\caption{Learning with Episodic Hypothesis Testing}
\label{alg:learning with hypothesis testing}
\begin{algorithmic}[1]
\State \textbf{Input:} 
    \State $\xi \in (0, 1)$.%: exploration parameter
    \State $f_i: \mathbb{R} \to \mathbb{R}_{+}$ and is an increasing function. % increasing function mapping player $i$'s utility to their exploration probability
    \State $\T \geq \frac{4}{(d-\tau)^2}\,\ln\bigl(\frac{1}{\xi^{\bar{r}}}\bigr)$, where $\bar{r} = \max_{\pi\in \Delta} \sum_{i \in I} f_i(\U{i}{\pi}) + 1$
    \State $\ptest = 1/\T + \pc$ for some $\pc \in (0,1)$.
\vspace{0.2cm}
\State \textbf{Initialization:}
each player $i$ holds a belief $b^0_i \in \mathcal{B}_i$ and an $\epsilon$-best response strategy $\pi^0_i = \Br^{\sigma}_i(b_i)$
\For{epoch $k = 1,2,\cdots$} 
    % \For{$t = 1,\cdots ,|I| \cdot \T$}
     \State each player $i \in i$ plays the game with strategy $\pi^k_i$ for $\T$ periods: $(a^t_i) \sim \pi^k_i$ for ${t = 1,\cdots, \T}$, and observe full action profiles $(a^t)_{t = 1,\cdots , \T}$
        \For{each player $i = 1, \cdots, |I|$}
            % \If{end of epoch ($t \mod |I| \cdot \T = 0$)}
                \State \parbox[t]{\dimexpr\linewidth - 1in}{with probability $\ptest$, conducts a hypothesis test against $b^k_i$ using observations $(a^t_{-i})_{t = 1,\cdots , \T}$.}
                % from $t = (i-1)\cdot \T$ to $t = i\cdot \T-1$ (total $\T$ periods): 
                % $(a^{(i-1)\cdot \T}, a^{(i-1)\cdot \T+1}, \cdots, a^{i\cdot \T-1})$.}
                    \If{rejects null hypothesis}
                    \State \parbox[t]{\dimexpr\linewidth - 1in}{sample $b^{k+1}_i$ uniformly from $\mathcal{B}_i$, $\pi^{k+1}_i = \Br^{\sigma}_i(b^{k+1}_i)$}
                    \ElsIf{fails to reject null hypothesis}
                    \State \parbox[t]{\dimexpr\linewidth - 1in}{with probability $\xi^{f_i(\U{i}{\pi_i,b_i})}$, sample $b^{k+1}_i$ uniformly from $\mathcal{B}_i$, $\pi^{k+1}_i = \Br^{\sigma}_i(b^{k+1}_i)$}
                    \Else
                    \State {$b^{k+1}_i = b^k_i, \pi^{k+1}_i = \pi^k_i$}
                    \EndIf
                    
            % \EndIf
        \EndFor
    % \EndFor
\EndFor
\end{algorithmic}
\end{algorithm}

We now provide more details on the key quantities of the learning algorithm: 
\begin{itemize}
    \item $\xi \in (0,1)$ is a hyperparameter that affects the epoch length, players' probability of conducting a hypothesis test, hypothesis test significance level, and probability of exploration.
    \item $\bar{r} = \max_{a \in A} \sum_{i \in I} u_i(\pi) + 1$ is a constant larger than the maximum total utility of all players in the game. The constant $\bar{r}$ determines the test significance level $\xi^{\bar{r}}$ in each epoch.
    \item $T(\xi^{\bar{r}})$ is the length of each epoch, which is also the sample size of each hypothesis test. Following from Proposition \ref{prop: hypothesis test}, $T(\xi^{\bar{r}}) \geq \frac{4}{(d-\tau)^2}\,\ln\bigl(\frac{1}{\xi^{\bar{r}}}\bigr)$ ensures that the hypothesis test conducted by each player has Type I and Type II errors upper bounded by $\xi^{\bar{r}}$.
    \item $\gamma(\xi) = 1/T(\xi^{\bar{r}}) + \gamma_0$ is the probability that each player conducts a test in each epoch, where $\gamma_0>0$ is the minimum test probability. As $\xi$ decreases, the epoch length $T(\xi^{\bar{r}})$ increases, and the probability of starting a test $\gamma(\xi)$ decreases. 
    \item $f_i: \mathbb{R} \to \mathbb{R}_{>0}$ is an increasing function that maps player $i$'s utility to a positive value. When player $i$'s hypothesis test fails to reject in epoch $k$, the player explores (resamples a new belief) with probability $\xi^{f_i(U_i(a_i^k, b_i^k))}$, where $U_i(a_i^k, b_i^k)$ is the expected utility of player $i$ given their belief and smoothed best response. Since $\xi \in (0,1)$ and $f_i(\cdot)$ is increasing, the exploration probability is higher when the utility $U_i(a_i^k, b_i^k)$ is low. The function $f_i(\cdot)$ can be viewed as player $i$'s sensitivity function, governing how their exploration probability changes with their utility, and may differ for different players.
\end{itemize}




% \paragraph{Key Insights:}
% \begin{itemize}
%     \item \textbf{Episodic structure}: The algorithm separates learning into distinct epochs, allowing players to stabilize strategies within each epoch before evaluating and updating beliefs.
%     \item \textbf{Controlled exploration}: The probability of testing and the sampling behavior balance the trade-off between learning from new observations and exploiting current beliefs.
%     \item \textbf{Incorporation of utility feedback}: Players are more likely to explore alternative beliefs if their observed utilities are unsatisfactory.
% \end{itemize}


A key feature of the learning dynamics is the integration of statistical hypothesis testing with adaptive, utility-sensitive exploration. The hypothesis test rigorously evaluates whether player $i$'s belief $b_i^k$ is within $\tau$ distance to the observed strategy profile $\pi_{-i}$. Specifically, when the test rejects the null hypothesis with significance level $\xi^{\bar{r}}$, it indicates with high confidence (controlled Type I error upper bound) that the discrepancy $\|\pi_{-i} - b_i^k\|_2 > \tau$; in this case, belief inconsistency is systematically excluded because player will resample a new belief with probability 1. Conversely, when the null hypothesis fails to be rejected, it indicates that $b_i^k$ is $\tau$-consistent with $\pi_{-i}$ with high probability (controlled Type II error). In this scenario, belief resampling only occurs when the player explores with probability $\xi^{f_i(U_i(a_i^k, b_i^k))}$, where $f_i(\cdot)$ encodes the player's sensitivity to utility dissatisfaction. The integration of statistical hypothesis testing and utility-sensitive exploration ensures that the learning process corrects significantly inconsistent beliefs while allowing adaptive exploration when current utility is unsatisfactory.



%A central feature of the learning dynamics is the integration of statistical hypothesis testing with adaptive, utility-sensitive exploration. Each player systematically tests the consistency of their belief $b_i^k$ against empirical observations of opponents’ strategies using a formal statistical test. This ensures that belief updates are made only when there is statistically significant evidence of inconsistency, thereby controlling Type I and Type II errors and avoiding overreactive strategy shifts due to limited data. Complementing this, the exploration mechanism is calibrated via a player-specific function $f_i(\cdot)$ that maps observed utility levels to exploration probabilities $\xi^{f_i(U_i(a_i^k, b_i^k))}$. This design allows players to dynamically modulate their propensity to explore new beliefs based on dissatisfaction with current performance, introducing a form of utility-dependent inertia into the learning process. Together, these mechanisms provide a robust balance between conservatism and adaptiveness: players retain stability through hypothesis testing, while the utility-driven exploration ensures responsiveness to suboptimal outcomes, even when the null hypothesis is not rejected. This dual approach enables convergence towards equilibria in dynamic and noisy environments where precise observations and fully rational behavior cannot be assumed.


% This framework supports the convergence of players' beliefs and strategies over time while incorporating robustness to incorrect initial beliefs and limited observation windows.

% In this section, we present a learning algorithm such that the strategy profile will concentrate on a specific set of $\epsilon$-Nash equilibria. 
% The algorithm operates in epochs. Within each epoch, players repeatedly sample actions based on their current strategy $\pi_i$. At the end of each epoch, players may conduct a hypothesis test on their beliefs using observations from the current epoch. If the null hypothesis is rejected, indicating that the belief is far from the true strategy profile, the player selects a new belief uniformly from the set of possible beliefs and updates their strategy accordingly. If the null hypothesis is failed to be rejected, the player may still explore new strategies with a probability determined by an exploration rate and their utility. 
% % For each player $i \in I$, let $\Br^{\sigma}_i: B_i \to \Delta_i$ be a best response function that maps any belief $b_i$ to an $\epsilon$-best response strategy $\pi_i = \Br^{\sigma}_i(b_i)$ in the discretized strategy simplex. 

% For each player $i \in I$, their hypothesis test has sample size $\T$. For any belief $b_i \in \mathcal{B}_i$, and true strategy profile $\pi_i \in \Delta_{-i}$, denote the type I error rate by $\alphai$ and type II error rate by $\betai$. Furthermore, 
% \begin{align}\label{eq: bound on alpha and beta}
%     \alphai \leq \xi^{\bar{r}}, \quad \betai \leq \xi^{\bar{r}}.
% \end{align} 
% Existence of such tests are guaranteed by proposition \ref{prop: hypothesis test}. For each player $i \in I$, let $f_i: \mathbb{R} \to \mathbb{R}^+$ be any increasing function.


% \ruifan{allowing every player to test deterministically or test with some probability?}
% \ruifan{leads to different stochastically stable states. deterministic testing leads to maximizing total utility while probabilistic testing leads to maximizing minimum utility.}


% \begin{algorithm}[H]
% \caption{Learning with episodic hypothesis testing}
% \label{alg:learning with hypothesis testing}
% \begin{algorithmic}[1]
% \State \textbf{Input:} 
%     \State $\xi$: exploration rate
%     \State $f_i$: increasing function mapping player $i$'s utility to their exploration probability
%     \State $\T$: length of hypothesis tests
%     \State $\ptest$: probability of conducting a test at the end of each epoch. 

% \State \textbf{Initialization:}
% Each player $i$ holds a belief $b_i\in \prod_{j \neq i} \Delta^M_j$ and an $\epsilon$-best response strategy $\pi_i = \Br^{\sigma}_i(b_i)$
% \For{epoch $k = 1,2,\cdots$}
%     \For{$t = 1,\cdots ,|I| \cdot \T$}
%     % sample new state from action profile
%         \For{each player $i = 1, \cdots, |I|$}
%             \State sample an action $a_i^t$ from current strategy $\pi_i$
%             \If{end of epoch ($t \mod |I| \cdot \T = 0$)}
%                 \State \parbox[t]{\dimexpr\linewidth - 1in}{with probability $\ptest$, conducts a hypothesis test against current belief $b_i$ using observations from $t = (i-1)\cdot \T$ to $t = i\cdot \T-1$ (total $\T$ periods): $(a^{(i-1)\cdot \T}, a^{(i-1)\cdot \T+1}, \cdots, a^{i\cdot \T-1})$.}
%                 %$(a^{t-\T}, a^{t-\T+1}, \cdots, a^{t})$.}
%                     \If{rejects null hypothesis}
%                     \State \parbox[t]{\dimexpr\linewidth - 1in}{chooses a new belief $b_i$ uniformly from $B_i$, and changes strategy accordingly $\pi_i = \Br^{\sigma}_i(b_i)$}
%                     \ElsIf{fails to reject null hypothesis}
%                     \State \parbox[t]{\dimexpr\linewidth - 1in}{explores with probability $\xi^{f(\U{i}{(\pi_i,b_i)})}$: player $i$ chooses a new belief $b_i$ uniformly from $B_i$, and changes strategy accordingly $\pi_i = \Br^{\sigma}_i(b_i)$}
%                     \EndIf
%                 \EndIf
%         \EndFor
%     \EndFor
% \EndFor
% \end{algorithmic}
% \end{algorithm}

% \ruifan{is there a difference: exploring at the end of a test vs explore at every epoch?}
% \ruifan{condition for $\ptest$: $\lim_{\xi \to 0} \ptest > 0$, $\lim_{\xi \to 0} 1-\ptest > 0$.}

% \ruifan{is there a difference: start a test and observe for T period, or start a test using recent T observation. The difference is in the first one, testing observations do not overlap (no dependency). Does the second one solve the infinite testing sample issue in lemma 2.}


% In the learning process described above, each player conducts a hypothesis test and (possibly) change their hypothesis and strategy every $\T$ timestep. For each player $i$ with belief $b_i$ and strategy $\pi_i = \Br^{\sigma}_i(b_i)$, their hypothesis test has null hypothesis $H_0: b_i = \pi_{-i}$, and alternative hypothesis $H_1: b_i \neq \pi_{-i}$. Each hypothesis test uses $\T$ samples from the observed action profile in the past $\T$ period. 

% In each epoch of the learning algorithm, players belief profile $b$ and strategy profile $\pi$ stays the same. For each player $i$, the reject region of their hypothesis test depends on their belief $b_i$, and the outcome of their hypothesis test depends on the realized action profiles observed within the epoch. Since the action profiles are sampled from the strategy profile \(\pi\), the transition of each player's belief only dependent on their belief $b_i$ and the strategy profile \(\pi\) of the current epoch. Given that each hypothesis test use a distinct subset of the data, the results of these tests are independent. Therefore, the transition of belief and strategy profiles at the end of each epoch only depend on the belief and strategy profile at the beginning of each epoch. This constitutes a Markov process on states $(b, \pi)$. 

% \manxi{Before proposition, make it clear that you are keeping track of the tuple of belief and strategy for k, which you call the state ofthe  Markov chain. This is a Markov chain with finite state space, and it has a unique stationary distribution (this can be a lemma).} \ruifan{done}


%Each state $z = (b, \pi) \in \mathcal{Z}$ consists of a belief profile $b = (b_1, \ldots, b_{|I|})$ and a corresponding smooth response strategy profile $\pi = (\pi_1, \ldots, \pi_{|I|})$.
% 's belief $b_i \in B_i$ and their strategy $\pi_i = \Br^{\sigma}_i(b_i) \in \Delta^M_i$. 

In the learning dynamics, for a belief \( b_i \in \mathcal{B}_i \), each player \( i \in I \) always selects their strategy \( \pi_i \in \Delta_i \) via the smooth best response function \( \pi_i = \Br_i^\sigma(b_i)\) with temperature parameter \( \sigma \). We refer to the tuple \((b, \pi)\), where \(b \in \mathcal{B}\) and \(\pi \in \Delta\) with \(\pi = \Br^\sigma(b_i)\), as the \emph{state} of the system. Given any $\xi > 0$, the learning process defines a Markov chain on the finite state space: 
\[\mathcal{Z}:= \{(b, \pi) \mid b_i \in \mathcal{B}_i,\, \pi_i = \Br^{\sigma}_i(b_i), \quad \forall i \in I\}.\] 

\begin{definition}[Consistent state]
A state \( z = (b, \pi) \in \mathcal{Z} \) is said to be \textit{consistent} if, for all players \( i \in I \), their belief \( b_i \) is within \(\tau\)-distance of the actual strategy profile \(\pi_{-i}\), where \(\pi\) is the smooth best response to \(b\). That is, the set of all consistent states is given by 
\[\Zdagger := \{z = (b, \pi) \in \mathcal{Z} \mid \|b_i - \pi_{-i}\|_2 \leq \tau, \quad \forall i \in I\}.\]
\end{definition}


\begin{assumption} \label{assump: sigma, tau, M}
Given any $\epsilon>0$, we assume that parameters $\sigma, \tau, M$ satisfy: 
\begin{subequations}
\begin{align}
    \sigma &\leq \frac{\epsilon}{2\cdot\log(\max_{i \in I}|A_i|)}, \quad  \tau \leq \frac{\epsilon \cdot \sigma}{2 \sqrt{|A|} \cdot (\max_{i \in I, a \in A} u_i(a))^2 \cdot (\max_{i \in I} |A_i| \cdot |A_{-i}|)} \label{eq: sigma and tau},\\
       M &\geq \frac{|I| \cdot \max_{i \in I} |A_{i}| }{\tau} \cdot \left( 1 + \frac{\sqrt{\max_{i \in I} |A_{i}|}}{\sigma} \cdot \max_{i \in I, a \in A} u_i(a) \cdot \max_{i \in I} |A_i||A_{-i}| \cdot |I| \right).  \label{eq: granularity M}
\end{align} 
\end{subequations}
\end{assumption}
Under assumption \ref{assump: sigma, tau, M}, each consistent state $z \in \Zdagger$ constitutes an $\epsilon$-Nash equilibrium. Proof is deferred to the appendix \ref{appendix: large M} to maintain the flow of the main text.
\begin{proposition}\label{lemma: sigma, tau, M}
    For any $\epsilon$, under Assumption \ref{assump: sigma, tau, M},
    the consistent state set $\Zdagger$ is non-empty. Furthermore, for any $z^{\dagger} = (b^{\dagger}, \pi^{\dagger}) \in \Zdagger$, $\pi^{\dagger}$ is an $\epsilon$-Nash equilibrium.
\end{proposition}
For each epoch $k$, we denote $z^k = (b^k, \pi^k)$ as the state at epoch $k$. The transition probability $P^{\xi}_{zz'}$ represents the likelihood of transitioning from state $z = (b,\pi)$ to state $z' = (b', \pi')$ in one epoch:
\[ P^{\xi}_{zz'} := \mathbb{P}(z^{k+1} = z' \mid z^k = z) \quad, \forall z, z' \in \mathcal{Z} \]


\begin{lemma}\label{lemma: P_ep}
    The Markov process described by transition $P^\xi$ has a finite state space and is aperiodic and irreducible for all $\xi \in (0, 1)$, and has a unique stationary distribution $\mu^{\xi}$.
\end{lemma}
The proof is deferred to Appendix \ref{appendix: transition matrix}.
A state is stochastically stable if it is in the support set of the stationary distribution $\mu^{\xi}(z)$. 

\begin{definition}
    A state $z \in \mathcal{Z}$ is \textit{stochastically stable} relative to the process defined by $P^\xi$ if \[\lim_{\xi \to 0} \mu_z^\xi > 0,\]
    where $\mu_z^{\xi}$ is the stationary distribution of state $z$.
\end{definition}

We assume that the strategy space for each player is sufficiently large. This guarantees that for each pair of players $i,j$, player $i$'s change in belief might potentially affect player $j$'s belief. We provide a verifiable sufficient condition for this assumption in Appendix \ref{appendix: bad strategy}.


\begin{assumption}\label{assump: bad strategy}
        For any player $i \in I$, and any consistent state
        $z = (b^z, \pi^z) \in \Zdagger$, there exists $\tilde{b}_i \in \Delta^M_{-i}$, and $\tilde{\pi}_i = \Br^{\sigma}_i(\tilde{b}_i)$ such that belief $\tilde{b}_i$ is at least $\tau$ distance away from strategy $\pi^z_{-i}$:
        \begin{align*}
            \|\tilde{b}_i - \pi^z_{-i}\|_2 > \tau,
        \end{align*}
        and strategy $\tilde{\pi}_i$ is at least $\tau$ distance away from belief $b^w_{ji}$ for any $j \neq i$ and any $b^w \in \prod_{i \in I} \Delta^M_{-i}$:
        \begin{align*}
            \|\tilde{\pi}_i -  b^w_{ji}\|_2 > \tau, \quad \forall j \neq i.
        \end{align*}
\end{assumption}


\begin{assumption}\label{assump: bad strategy}
        For any player $i \in I$, any belief profile $b^w \in \prod_{i \in I} \Delta^M_{-i}$, and any belief consistent state
        $z = (b^z, \pi^z) \in \Zdagger$, there exists $\tilde{b}_i \in \Delta^M_{-i}$, and $\tilde{\pi}_i = \Br^{\sigma}_i(\tilde{b}_i)$ such that belief $\tilde{b}_i$ is at least $\tau$ distance away from strategy $\pi^z_{-i}$:
        \begin{align*}
            \|\tilde{b}_i - \pi^z_{-i}\|_2 > \tau,
        \end{align*}
        and strategy $\tilde{\pi}_i$ is at least $\tau$ distance away from belief $b^w_{ji}$ for any $j \neq i$:
        \begin{align*}
            \|\tilde{\pi}_i -  b^w_{ji}\|_2 > \tau, \quad \forall j \neq i.
        \end{align*}
\end{assumption}

\begin{theorem} \label{theorem:main}
    A state $z = (b, \pi)$ is stochastically stable if and only if $z \in \Zdagger$, and \[\min_{i \in I} f_i(\U{i}{\pi}) = \max_{z' = (b', \pi') \in \Zdagger} \min_{i \in I} f_i(\U{i}{\pi'}).\]
    Consequently, for any $\epsilon > 0$, $\eta > 0$, there exists $\bar{\xi} > 0$ such that for all $0 < \xi < \bar{\xi}$, the strategy profile being played is an $\epsilon$-Nash equilibrium in which the minimum value of the function \( f_i(\U{i}{\pi}) \) over all players $i \in I$ is maximized, at least $1-\eta$ of the time.
\end{theorem}
Theorem \ref{theorem:main} states that a state \( z = (b, \pi) \) is stochastically stable if 
\begin{enumerate}
    \item Each player has a true belief about the other players' strategy, and
    \item The minimum value of the function \( f_i(\U{i}{\pi}) \) over all players $i \in I$ is maximized.
\end{enumerate}
When $f_i(\cdot)$ is the identity function for all player $i \in I$, a stochastically stable state achieves the best worst-case utility outcome. That is, the stochastically stable states are the ones where the worst pay-off player's utility is maximized over all belief-consistent states. It is easy to see that stochastically stable states are the only states that have nonvanishing probability when the parameter $\xi$ becomes arbitrarily small. In other words, the Markov process is in a stochastically stable state most of the time. Therefore, the actual strategy profiles being played are a $\epsilon$-Nash equilibrium that maximizes the minimum value of the function \( f_i(\U{i}{\pi}) \) over all players $i \in I$ is maximized.

\begin{corollary}
    When $f_i(x) = x$ for all players $i \in I$, the stochastically stable states correspond to the set of Nash equilibria that maximize the minimum utility across all players. Specifically, a state $z = (b, \pi)$ is stochastically stable if and only if $z \in \Zdagger$, and
    \[\min_{i \in I} \U{i}{\pi} = \max_{z' = (b', \pi') \in \Zdagger} \min_{i \in I} \U{i}{\pi'}.\]
\end{corollary}

% \textbf{Stochastic stability (Pradelski and Young 2012)} The set of \textit{stochastically stable states} $Z^*$ of the process $z(t)$ is the minimal subset of states such that, given any small $\alpha > 0$, there is a number $\xi_\alpha > 0$ such that whenever $0 < \xi \leq \xi_\alpha$, $z(t) \in \mathcal{Z}^*$ for at least $1 - \alpha$ of all periods $t$.

    % \textbf{Stochastic Stability (Young 1993)} A state $h \in H$ is \textit{stochastically stable} relative to the process $P^\xi$ if $\lim_{\xi \to 0} \mu_h^\xi > 0$.
% The Markov chain defined by $P^{\xi}$ is homogeneous because the transition probabilities $P^{\xi}_{zz'}$ depend only on the current state $z$ and not on the epoch $k$. This follows from our learning algorithm where:
% \begin{enumerate}
%     \item The probability of conducting a hypothesis test ($\ptest$) is constant across epochs.
%     \item The probability of rejecting the null hypothesis depends only on the current belief and strategy profiles.
%     \item The exploration probability $\xi^{f_i(\U{i}{\pi_i,b_i})}$ depends only on the current state.
%     \item The sampling of new beliefs is uniform from $\mathcal{B}_i$ and independent of the epoch.
% \end{enumerate}


% can write out the lower bound for the probability of transitions between states that the belief only differs in one player
% \[ P^{\xi}_{i, zz'}\cdot (1-\ptest)^{|I|-1} \leq P^{\xi}_{zz'} .\]
% Furthermore, for any two states $z, z'$, then 
% \[0 < (\ptest)^{|I|} \cdot \prod_{i \in I}\xi^{f_i(\U{i}{\pi_i,b_i})} \leq P^{\xi}_{zz'} \leq \min_{i \in I} P^{\xi}_{i, zz'}, \quad \forall i \in I.\]
% \[0 < P^{\xi}_{i, zz'} \cdot (\ptest)^{|I|-1} \cdot \prod_{j \neq i}\xi^{f_j(\U{j}{\pi_j,b_j})} \leq P^{\xi}_{zz'} \leq P^{\xi}_{i, zz'}, \quad \forall i \in I.\]
% Let $I_c$ be the set of players whose beliefs are consistent but changed. Let $I_d$ be the set of players whose beliefs are not consistent and changed.

% want to show that the resistance from $z$ to $z'$ greater than or equal to $\min_{i \in I_c} \xi^{f_i(\U{i}{\pi_i,b_i})}$.
% For all $r < \min_{i \in I_c} \xi^{f_i(\U{i}{\pi_i,b_i})}$, 
% \[0 \leq \lim_{\xi \to 0} P^{\xi}_{zz'}\cdot\xi^{-r_{i, zz'}} \leq blah = 0\]

% From the original proof, we have
% \begin{align*}
%     \lim_{\xi \to 0} P^{\xi}_{zz'}\cdot\xi^{-r_{i, zz'}}\leq  \lim_{\xi \to 0} P^{\xi}_{i, zz'}\cdot\xi^{-r_{i, zz'}} = \pc \cdot \frac{1}{|\mathcal{B}_i|} < \infty.
% \end{align*}
% Now I need to bound it above $0$:
% \[0 <\lim_{\xi \to 0} P^{\xi}_{zz'}\cdot\xi^{-r_{i, zz'}}\]

% It is difficult to verify condition $3$ of regular perturbation:



% \begin{lemma}\label{lemma: transition matrix}
% For any $\xi > 0$, $\tau > 0$, $z = (b,\pi), z' = (b', \pi') \in \mathcal{Z}$, the Markov chain transition probability $P^{\xi}_{zz'}$ is the product of individual transitions for each player $i \in I$:
% \begin{align*}
%     P^{\xi}_{zz'} = \prod_{i \in I} P^{\xi}_{i, zz'},
% \end{align*}where $P_{i, zz'}^{\xi}$
% is the probability of player $i$ updating their belief from $b_i$ to $b^{'}_i$. 
% % For each player $i \in I$, the transition probability $P^{\xi}_{i, zz'}$ can be written as follows:

% % When current belief matches others' strategies ($b_i = \pi_{-i}$):\\
% %     If $b'_i = b_i$:
% %     \begin{align} \label{eq: chain case1}
% %         P^{\xi}_{i, zz'} &= 1-\ptest + \notag \\
% %         &\ptest \cdot \left((1-\alphai)\cdot (1-\xi^{f_i(\U{i}{\pi_i,b_i})}) + \left((1-\alphai)\cdot \xi^{f_i(\U{i}{\pi_i,b_i})} + \alphai \right) \cdot \frac{1}{|B_i|}\right).
% %         \end{align}
% %     If $b'_i \neq b_i$:
% %     \begin{align}\label{eq: chain case2}
% %         P^{\xi}_{i, zz'} &= \ptest \cdot \left((1-\alphai)\cdot \xi^{f_i(\U{i}{\pi_i,b_i})} + \alphai \right) \cdot \frac{1}{|B_i|}.
% %     \end{align}
    
% %     When current belief differs from others' strategies ($b_i \neq \pi_{-i}$):\\
% %     If $b'_i = b_i$:
% %     \begin{align}\label{eq: chain case3}
% %         P^{\xi}_{i, zz'} &= 1-\ptest + \ptest \cdot \notag \\
% %         &\left(\betai(1-\xi^{f_i(\U{i}{\pi_i,b_i})}) + \left(\betai\xi^{f_i(\U{i}{\pi_i,b_i})} + (1-\betai)\right)\frac{1}{|B_i|}\right).
% %         \end{align}
% %     If $b'_i \neq b_i$:
% %     \begin{align} \label{eq: chain case4}
% %         P^{\xi}_{i, zz'} &= \ptest \cdot \left(\betai\xi^{f_i(\U{i}{\pi_i,b_i})} + (1-\betai)\right)\frac{1}{|B_i|}.
% %     \end{align}

% % \ruifan{use case environment}
% When current belief is close to others' true strategies ($\|b_i - \pi_{-i}\|_2 \leq \tau$):
% \begin{subnumcases}{P^{\xi}_{i, zz'} =}
%     1-\ptest + \ptest \cdot \left((1-\alphai)\cdot (1-\xi^{f_i(\U{i}{\pi_i,b_i})}) + \right.\notag \\
%     \left. \qquad \left((1-\alphai)\cdot \xi^{f_i(\U{i}{\pi_i,b_i})} + \alphai \right) \cdot \frac{1}{|B_i|}\right) & if $b'_i = b_i$ \label{eq: chain case1}\\
%     \ptest \cdot \left((1-\alphai)\cdot \xi^{f_i(\U{i}{\pi_i,b_i})} + \alphai \right) \cdot \frac{1}{|B_i|} & if $b'_i \neq b_i$ \label{eq: chain case2}
% \end{subnumcases}

% When current belief is far from others' true strategies ($\|b_i - \pi_{-i}\|_2 > \tau$):
% \begin{subnumcases}{P^{\xi}_{i, zz'} =}
%     1-\ptest + \ptest \cdot \left(\betai(1-\xi^{f_i(\U{i}{\pi_i,b_i})}) + \right. \notag\\
%     \left. \qquad \left(\betai\xi^{f_i(\U{i}{\pi_i,b_i})} + (1-\betai)\right)\frac{1}{|\mathcal{B}_i|}\right) & if $b'_i = b_i$ \label{eq: chain case3}\\
%     \ptest \cdot \left(\betai\xi^{f_i(\U{i}{\pi_i,b_i})} + (1-\betai)\right)\frac{1}{|\mathcal{B}_i|} & if $b'_i \neq b_i$ \label{eq: chain case4}
% \end{subnumcases}

% In the above expressions:
% \begin{itemize}
%     \item $\alphai$ : probability of rejecting null hypothesis when beliefs match strategies
%     \item $\betai$ : probability of rejecting null hypothesis when player $i$'s belief $b_i$ differ from other players' actual strategy profile $\pi_{-i}$
%     \item $|B_i|$ : size of player $i$'s belief space (for uniform sampling).
% \end{itemize}

% Furthermore, the Markov process $P^\xi$ has a finite state space and has a unique stationary distribution $\mu^{\xi}$.
% \end{lemma}
